Characterisation of silicon microstrip detectors for the ATLAS Phase-II Upgrade with a micro-focused X-ray beam

The planned HL-LHC (High Luminosity LHC) in 2025 is being designed to maximise the physics potential through a sizable increase in the luminosity up to 6*10^34 cm^-2 s^-1. A consequence of this increased luminosity is the expected radiation damage at 3000 fb^-1 after ten years of operation, requiring the tracking detectors to withstand fluences to over 1*10^16 1 MeV n_eq/cm^2 . In order to cope with the consequent increased readout rates, a complete re-design of the current ATLAS Inner Detector (ID) is being developed as the Inner Tracker (ITk). Two proposed detectors for the ATLAS strip tracker region of the ITk were characterized at the Diamond Light Source with a 3 um FWHM 15 keV micro focused X-ray beam. The devices under test were a 320 Um thick silicon stereo (Barrel) ATLAS12 strip mini sensor wire bonded to a 130 nm CMOS binary readout chip (ABC130) and a 320 Um thick full size radial (end-cap) strip sensor - utilizing bi-metal readout layers - wire bonded to 250 nm CMOS binary readout chips (ABCN-25). A resolution better than the inter strip pitch of the 74.5 um strips was achieved for both detectors. The effect of the p-stop diffusion layers between strips was investigated in detail for the wire bond pad regions. Inter strip charge collection measurements indicate that the effective width of the strip on the silicon sensors is determined by p-stop regions between the strips rather than the strip pitch.

==> Proofreading_for_JINST_065P_0316 <==
1. Abstract, second to last paragraph: please remove last sentence, as the section this sentence refers to was removed from the paper.

Old version: 
A resolution better than the inter strip pitch of the 74.5 μm strips was achieved for both detectors. The effect of the p-stop diffusion layers between strips was investigated in detail for the wire bond pad regions. The collected hits allowed for the identification of operating thresholds for both devices, making it possible to compare signal response between different versions of silicon strip detector modules.

New version:
A resolution better than the inter strip pitch of the 74.5 μm strips was achieved for both detectors. The effect of the p-stop diffusion layers between strips was investigated in detail for the wire bond pad regions.


2. page 1, Introduction, 3rd paragraph, last sentence: please add space \, between \pm and 2.5

Old version:
The detectors cover \unit[$\pm2.5$]{units of pseudorapidity}~\cite{2}.

New version:
The detectors cover \unit[$\pm\,2.5$]{units of pseudorapidity}~\cite{2}.


3. page 2, subsection ABCN-25 end-cap module, first paragraph, last sentence: correct number

Old version:
The circular shape of an end-cap leads to wedge shaped sensors with
strip pitches increasing towards outer radii from 67 μm to 106 μm [10].

New version:
The circular shape of an end-cap leads to wedge shaped sensors with
strip pitches increasing towards outer radii from 93 μm to 106 μm [10].


4. page 3, subsection ABC130 mini module, third paragraph, last sentence: correct number

Old version:
The mini sensors under test consisted of 256 strips (74.5 μm pitch in 2 rows) with punch through protection (PTP) structures and an overall size of 1 × 1 cm 2 .

New version:
The mini sensors under test consisted of 104 strips (74.5 μm pitch in 2 rows) with punch through protection (PTP) structures and an overall size of 1 × 1 cm 2 .


5. page 5, subsection DAQ and readout, last paragraph: change singular to plural

Old version:
All data were written to disk by the DAQ as custom histograms, and analysis scripts written in ROOT to study signal response at various positions and thresholds.

New version:
All data were written to disk by the DAQ as custom histograms, and analysis scripts written in ROOT to study signal responses at various positions and thresholds.


6. page 8, subsection effective strip width, second to last paragraph, last sentence: change singular to plural

Old version:
The width of the detection range match the strip pitch of the sensor, as expected.

New version:
The width of the detection range matches the strip pitch of the sensor, as expected.


7. page 9, figure 7a, caption, first sentence: typo

Old version:
inidividual

New version:
individual

